Keep Doing What Worked: Behavioral Modelling Priors for Offline Reinforcement Learning

Off-policy reinforcement learning algorithms promise to be applicable in settings where only a fixed data-set (batch) of environment interactions is available and no new experience can be acquired. This property makes these algorithms appealing for real world problems such as robot control. In practice, however, standard off-policy algorithms fail in the batch setting for continuous control. In this paper, we propose a simple solution to this problem. It admits the use of data generated by arbitrary behavior policies and uses a learned prior -- the advantage-weighted behavior model (ABM) -- to bias the RL policy towards actions that have previously been executed and are likely to be successful on the new task. Our method can be seen as an extension of recent work on batch-RL that enables stable learning from conflicting data-sources. We find improvements on competitive baselines in a variety of RL tasks -- including standard continuous control benchmarks and multi-task learning for simulated and real-world robots.

==> deprecated.tex <==

$Q^{\pi_k}$ here represents the expected discounted cumulative reward for a target task (represented by reward $r$) when following $\pi_k$ i.e.: $Q^{\pi_k}(s_t, a_t) = \mathbb{E}_{\pi_k}[\sum_{i=t}^\infty r(s_i, a_i) | a_i \sim \pi_k, s_{i + 1} \sim p(\cdot | s_i, a_i) ]$.
Note that when performing offline RL from a batch of data $\mathcal{D}$ the \textbf{reward $r$ might be computed post-hoc and does not necessarily correspond to the reward optimized by the behavior policy $\mu$} from which the data was collected. That is $Q^{\pi_k}$ must be estimated off-policy in our setting.
% In the MPO algorithm \citep{abdolmaleki2018maximum}, this hard KL constraint is achieved by Lagrangian relaxation  $\lambda$ is adaptively optimized to achieve an average KL of $\epsilon$.
We aim to solve this optimization problem by employing the MPO algorithm for policy optimization \citep{abdolmaleki2018maximum} -- and assume that we learn $Q^{\pi_k}$ alongside from off-policy data. Note that other RL algorithms could be used in the following, as long as they allow us to penalize a distance to a prior policy (though in practice we found it especially useful to be able to express this penalty via a hard-constraint as in MPO). 
In the original MPO algorithm, policy optimization occurs in a policy improvement loop. First $Q^{\pi_k}$ is learned and then $\pi_{k+1}$ is found by setting $\pi_{\text{prior}}$ to 
the last policy ($\pi_\text{prior} = \pi_k$) in order to allow slow convergence to the optimal policy (while preventing premature convergence). Our method is to, instead, set this prior to a new distribution representing actions observed in the data.

The first prior we consider is a prior that simply aims to represent the behavior policy itself. This is similar to the approach of BEAR-QL \citep{kumar2019stabilizing}, but while they utilize a non-parametric representation of the behavior policy (and then minimize the sampled maximum mean discrepancy instead of a KL), we instead learn a parameteric behavioral cloning policy $\pibc$ by minimizing the negative log likelihood of observed data:
\begin{equation}
\pi_\text{prior} = \arg \min_{\pibc} \mathbb{E}_{(s,a)\sim\mathcal{D}} \left[ - \log \pibc(a|s) \right],
\end{equation}
where $\mathcal{D}$ is the fixed dataset of transitions used for learning.

While regularizing towards the behavior policy helps to prevent the use of unobserved actions, it may also prevent the policy from improving on the behavior. Specifically, if $\mathcal{D}$ contains both good and bad behaviors, regularizing toward $\pibc$ will move us toward both the good and bad actions taken. While this may be acceptable for datasets consisting entirely of expert demonstrations (or data that is at least dominated by successful trajectories), we often want to learn from datasets containing behaviors whose trajectories are imperfect for the task being learned. In particular, we are interested in the case where we have a dataset collected from imperfect (online learning) data for multiple tasks. Clearly, for any given target task (specified via a reward) that we aim to learn from this data, such a source of data will contain a diverse set of trajectories -- both (partially) successful and actively harmful for the target task.

With this in mind, we propose the class of advantage-weighted behavioral cloning priors, $\piawbc$, which bias the RL policy to ``keep doing what worked'' and are learned by minimizing:
\begin{equation}
\pi_\text{prior} = \arg \min_{\piawbc} \mathbb{E}_{(s,a)\sim\mathcal{D}} \left[ -\log \piawbc(a|s) f(A^{\pi_k}(s, a)) \right],
\label{eq:awbc}
\end{equation}
where $f$ is a monotonically increasing nonnegative function, and $A^{\pi_k}$ is the action advantage function (for the target task) wrt. the current policy $\pi_k$. This objective still tries to maximize the log likelihood of observed actions, and therefore avoids taking actions not supported by data. However, by weighting actions by a monotonic function of advantage, we focus more heavily on copying "good" actions while ignoring poor actions. Thus, while $\pibc$ learns to keep doing everything that $\mu$ did, $\piawbc$ learns to keep doing what worked (and only what worked).

For simplicty -- to keep the number of hyperparameters to a minimum while keeping the prior broad -- we let $f=1_+$ (the unit step function). We note that in general \eqref{eq:awbc} is a form of transformed policy gradient, though it is not unbiased and will thus not necessarily converge to the optimal policy in itself (due to the missing importance weighting and dependent on the form of $f$). It should be noted that this bias is not necessarily harmful, but is desired, in order to prevent the policy trained with this prior from taking actions unsupported by data. We also note that we tried several different functions for $f$ including exponentiation and hard sigmoid with finite slope, but found that choice of function did not make a significant difference to final policy performance.
